Deceptive Semantic Shortcuts on Reasoning Chains: How Far Can Models Go without Hallucination?

Despite the recent advancement in large language models (LLMs) and their high performances across numerous benchmarks, recent research has unveiled that LLMs suffer from hallucinations and unfaithful reasoning. This work studies a specific type of hallucination induced by semantic associations. Specifically, we investigate to what extent LLMs take shortcuts from certain keyword/entity biases in the prompt instead of following the correct reasoning path. To quantify this phenomenon, we propose a novel probing method and benchmark called EureQA. We start from questions that LLMs will answer correctly with utmost certainty, and mask the important entity with evidence sentence recursively, asking models to find masked entities according to a chain of evidence before answering the question. During the construction of the evidence, we purposefully replace semantic clues (entities) that may lead to the correct answer with distractor clues (evidence) that will not directly lead to the correct answer but require a chain-like reasoning process. We evaluate if models can follow the correct reasoning chain instead of short-cutting through distractor clues. We find that existing LLMs lack the necessary capabilities to follow correct reasoning paths and resist the attempt of greedy shortcuts. We show that the distractor semantic associations often lead to model hallucination, which is strong evidence that questions the validity of current LLM reasoning.

==> content/tables/openSourceModel.tex <==
\begin{table*}[h]
\centering
\label{table:methods}
{
\begin{tabular}{@{}cccccccccccccc@{}} % l for left-aligned, c for centered
\toprule
% difficulty row
% \multicolumn{11}{c}{\texttt{hard}} & \multicolumn{2}{c}{\texttt{easy}}\\
% \cmidrule(l){2-11}\cmidrule(l){12-13}
% depth row
depth &\multicolumn{2}{c}{\texttt{d}=1} & \multicolumn{2}{c}{\texttt{d}=2} & \multicolumn{2}{c}{\texttt{d}=3} & \multicolumn{2}{c}{\texttt{d}=4} & \multicolumn{2}{c}{\texttt{d}=5} \\ 
\cmidrule(r){2-3} \cmidrule(lr){4-5} \cmidrule(l){6-7} \cmidrule(l){8-9} \cmidrule(l){10-11} % Rules under the subheaders
% prompt row
& \textit{direct} & \textit{icl} & \textit{direct} & \textit{icl} & \textit{direct} & \textit{icl} & \textit{direct} & \textit{icl} & \textit{direct} & \textit{icl}\\ % Subheaders
\midrule
Llama-2-7b & 29.5   & 22.0   & 21.4   & 11.9   & 15.8   & 13.0   & 10.6   & 11.3   & 10.9   & 14.5   \\
Llama-2-13b & 40.0   & 28.5  & 27.0   & 16.4   & 20.5   & 15.8   & 11.3   & 15.9   & 13.9   & 19.4   \\
Llama-2-70b & 45.0   & 57.0   & 24.5   & 35.2   & 17.8   & 39.0   & 18.5   & 32.5   & 12.1   & 34.5   \\
\bottomrule
\end{tabular}
}
\caption{Accuracy of Llama-2 models across different depths \texttt{d} of reasoning (number of layers in the questions). We evaluate two prompt strategies: \textit{direct} zero-shot prompt and \textit{icl} with two examples. The 7b and 13b versions are chat variants and the 70b version is instruct variant.}

\label{table:llamaRes}
\end{table*}
